Shape and Material Capture at Home

In this paper, we present a technique for estimating the geometry and reflectance of objects using only a camera, flashlight, and optionally a tripod. We propose a simple data capture technique in which the user goes around the object, illuminating it with a flashlight and capturing only a few images. Our main technical contribution is the introduction of a recursive neural architecture, which can predict geometry and reflectance at 2^{k}*2^{k} resolution given an input image at 2^{k}*2^{k} and estimated geometry and reflectance from the previous step at 2^{k-1}*2^{k-1}. This recursive architecture, termed RecNet, is trained with 256x256 resolution but can easily operate on 1024x1024 images during inference. We show that our method produces more accurate surface normal and albedo, especially in regions of specular highlights and cast shadows, compared to previous approaches, given three or fewer input images. For the video and code, please visit the project website http://dlichy.github.io/ShapeAndMaterialAtHome/.

==> teaser.tex <==
% teaser.tex is referenced in cvpr.cls
\newcolumntype{Y}{>{\centering\arraybackslash}X}
\includegraphics[width=.95\textwidth]{teaser2.png}
\vspace{-2em}
%\captionof{figure}{The right-hand side shows a minimal capture setup using just an Iphone, flashlight and sweet potato in lieu of a tripod. The right-hand side top row shows the estimated normals, albedo and roughness. The bottom row shows the mesh reconstructed and rendered with the estimated albedo and roughness, the same reconstruction from a novel view, and the mesh rendered with uniform albedo.}
\captionof{figure}{A bare-bones capture setup (left) consisting of only an iPhone, a flashlight and a sweet potato. The user captures a few images (with voice control) of the object by moving around with a flashlight directed at the object. We then reconstruct surface normal, albedo and roughness at high-resolution (1024$\times$1024). Normals are integrated to create a mesh that is rendered with novel views and illuminations.}
\label{fig:teaser}



% \begin{strip}\centering
% \includegraphics[width=0.98\linewidth]{latex/figures/teaser2.png}
% \captionof{figure}{The right-hand side shows a minimal capture setup using just an Iphone, flashlight and sweet potato in lieu of a tripod. The right-hand side top row shows the estimated normals, albedo and roughness. The bottom row shows the mesh reconstructed and rendered with the estimated albedo and roughness, the same reconstruction from a novel view, and the mesh rendered with uniform albedo.
% \label{fig:teaser}}
% \end{strip}
